Equitable non-contact infrared thermography after solar loading using deep learning

Widely deployed for fever detection, infrared thermometers (IRTs) enable rapid non-contact measurement of core body temperature but are inaccurate in unconstrained environments when skin temperature is transient. In this work, we present the first study on the effect of solar loading--solar radiation-induced elevation of skin but not core temperature--on IRT performance. Solar loading causes poor specificity in IRT fever detection, and the standard procedure is to reacclimate subjects for up to 30 minutes before IRT measurement. In contrast, we propose a single-shot deep learning model that removes solar loading transients from thermal facial images, allowing accurate IRT operation in solar loaded conditions. Forehead skin temperature increases by 2.00{\deg}C after solar loading, and our deep learning model, SL-Net, reduces this error by 68\% to 0.64{\deg}C. We show that the solar loading effect depends on skin tone, introducing inequity in IRT performance, while SL-Net is unbiased. We open source a diverse dataset of 100 subjects with co-registered RGB-thermal images, and IRT and skin tone measurements. Our work shows that it is possible to use machine learning to correct complex thermal perturbations to enable robust and equitable human thermography.

==> sections/dump.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lccccccccccccc} \toprule
    & \multicolumn{12}{c}{Forehead Error (°C)} \\
    \cmidrule(lr){2-13}
    & \multicolumn{3}{c}{MAE ($\downarrow$)} & \multicolumn{3}{c}{MSE ($\downarrow$)} & \multicolumn{3}{c}{RMSE ($\downarrow$)} & \multicolumn{3}{c}{MAPE ($\downarrow$)} \\ 
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
    Model & Base & Solar & Mean  & Base & Solar & Mean  & Base & Solar & Mean  & Base & Solar & Mean \\
    \midrule
    No correction & \best{0} & 1.999 & 1.000 & \best{0} & 4.889 & 2.444 & \best{0} & 2.211 & 1.106 & \best{0} & 0.059 & 0.030 \\
    Ours (Exp Fit) & 0.361 & 1.380 & 0.871 & 1.222 & 2.408 & 1.815 & 1.105 & 1.552 & 1.329 & 0.011 & 0.041 & 0.026 \\
    Ours (MLP) & 0.354 & 0.700 & 0.527 & 0.199 & 0.661 & 0.430 & 0.446 & 0.813 & 0.630 & 0.010 & 0.021 & 0.016 \\
    Ours (ResUNet) & 0.216 & 0.656 & 0.436 & 0.113 & 0.593 & 0.353 & 0.336 & 0.770 & 0.553 & 0.006 & \best{0.019} & 0.013 \\
    Ours (ResUNet + Classifier) & 0.047 & \best{0.638} & \best{0.343} & 0.043 & \best{0.581} & \best{0.312} & 0.208 & \best{0.762} & \best{0.485} & 0.001 & \best{0.019} & \best{0.010} \\
    \bottomrule
    \end{tabular}
    \caption{
    \textbf{All three of our models improve solar loading reconstruction across all metrics.} Our final model improves solar loading error by 68\%. (todo: add model size, \# params)
    }
    \label{tab:forehead_results}
\end{table*}



==> sections/related-works.tex <==
In this work, we aim to improve human infrared thermography by studying skin tone bias and correcting solar loading errors in a physically-constrained manner. 
We first review studies on infrared thermography and skin tone biases in remote health sensing.
We then discuss general efforts to incorporate physics into machine learning models and specific applications to health sensing.

\subsection{Infrared Thermography}
Infrared thermometers detect fevers by measuring skin temperature increase during febrile states. Due to the rise in IRT usage during the COVID-19 pandemic, questions have been raised about the accuracy and biases of the devices. \cite{Adams2021} found that age and gender affect IRT accuracy.
Studies on skin tone bias have conflicting conclusions.
\cite{Khan2021} compared IRT results across human-annotated skin tone categories: light, medium and dark. No skin tone bias was found, although the dataset was heavily skewed towards light skin.
\cite{Strasse2022} compared the performance of IRTs across
measurement locations and ethnic groups (Black, White and mixed). Again, no bias was found.
However, \cite{Bhavani2022} showed that IRTs, specifically temporal artery thermometers, underestimate temperature in Black patients. Participants were grouped by self-reported ethnicity (Black and White). The authors hypothesized that this bias is caused by different thermal emissivities in darker skin, but \cite{Charlton2020} show that skin pigmentation does not affect emissivity.
These conflicting studies show that race, ethnicity and subjective skin tone labeling preclude an understanding of bias in IRTs.

\paragraph{Lack of Solar Loading Studies}
IRTs measure hot areas of the face to be robust to environmental effects, but they are still are inaccurate when the ambient temperature deviates from room temperature \cite{Spindel2021, Erenberk2013, Dzien2020, Ogawa2022, Ravi2022, Tay2015}. Recent works improve IRT operation in different environmental conditions by fitting relevant temperature variables to a linear function  \cite{Shajkofci2022, Qiu2023}. 
To the best of our knowledge, these are no prior works that study or correct solar loading error in IRTs. 


\subsection{Bias in Health Sensing}
Seminal work by \cite{Buolamwini2018} revealed racial and gender disparities in computer vision algorithms. 
Unfortunately, biases arise in other technologies, such as optical health sensing devices. Optical biases arise when the light transport is inadequately characterized for certain groups, such as people with dark skin \cite{Kadambi2021}.
For example, pulse oximeters and remote photo-plethysmography, which measure blood oxygenation and heart rate respectively, are known to perform worse for darker skin tones due to poor signal-to-noise ratio \cite{Nowara2020, Sjoding2020}.
Biases can be resolved computationally by balancing skin tones in a dataset with synthetic data, or physically by using multi-modal data \cite{Wang2022, Vilesov2022}. 

==> sections/theory.tex <==
\newcommand{\vecx}{\mathbf{x}}

% The key principle in infrared thermography is that skin temperature increases with body temperature, allowing non-contact detection of fevers. 
% Skin temperature is influenced by external factors, such as solar radiation, that break down the traditional method of thermography.

Skin temperature depends on core body temperature and under specific conditions, the relationship between the two variables is known. Infrared thermometers leverage this relationship to estimate body temperature in a non-contact manner but when the specified conditions are not met, the results can vary widely from the ground truth. 
The relationship between skin and body temperature is derived from the \textit{bioheat equation}. When solar radiation is included as a heat source in the bioheat equation, we can understand how to computationally correct solar loading.


\subsection{Skin Temperature}
Skin temperature is a complex function of endogenous (blood perfusion, metabolism and core conduction) and exogenous (convective and radiative) heat sources.
The balance of heat sources determines skin temperature and is described by \textit{Pennes bioheat equation} \cite{Wissler1998} \cite{Hristov2019}. The bioheat equation describes a 3D distribution of skin and tissue temperature, $u(\vecx, t)$, as a partial differential equation:
\begin{align}
    \rho c \pdv{u}{t} 
    = k \nabla^2 u 
    + b(\vecx) (T_c - u) 
    + q_m
    + q_\text{ext}(\vecx), \label{eq:gov}
\end{align}
where $\rho, c, k$ are skin density, heat capacity and thermal conductivity, and $q_m$ and $q_\text{ext}$ are metabolic and external heat. 
Blood flow is defined as $b = \rho_b c_b v_b$, where $\rho_b, c_b, v_b$ are blood density, specific heat and flow rate. 
At the skin surface, flux from the environment—air radiation and convection—must equal flux from the skin:
\begin{equation}
    k \pdv{u}{z}\biggr\rvert_{z=0} 
    = h\,(u(z\!=\!0) - T_e),
    \label{eq:boundary-condition}
\end{equation}
where $h$ is the combined radiative and convective coefficient (which includes skin emissivity, $\varepsilon$) and $T_e$ is the air temperature. 


\subsubsection{Temperature States}
Skin temperature can be stationary or transient, depending on the environment. 
Infrared thermography assumes that skin temperature is stationary and that subjects are acclimated to ``normal" indoor conditions ($T_e = 21^\circ C$, relative humidity=$70\%$). 
We call this the \textit{baseline} state, denoted by $u_0(\vecx)$. 
In this work, we are interested in removing deviations from the baseline temperature induced by solar radiation.
As such, we decompose skin temperature as the sum of the baseline, $u_0$, and transient, $s$, components:
\begin{equation}
    u(\vecx, t) = u_0(\mathbf{x}) + s(\mathbf{x},t).
\end{equation}
$u_0$ is found by solving \Cref{eq:gov} when $q_\text{ext} = 0$ and $\pdv{u}{t} = 0$. During the baseline state, the relationship between skin and body temperature is known [cite].

\subsubsection{Relating Skin Temperature to Body Temperature}
explain how IRTs convert Tskin to Tbody.

\subsection{Skin Color}
Chromophores in the skin—hemoglobin and melanin—determine how skin interacts with light. Skin absorption of light determines skin color (in visible light) and skin temperature (in infrared), and the population has varying concentrations of chromophores. The capacity for absorption is given by the absorption coefficient, $\mu_a$.

The skin absorption coefficient is the sum of the melanin-free epidermal absorption, $\mu_{a,\text{epi}}$, and
melanin absorption, $\mu_{a,\text{mel}}$ \cite{Jacques2013}:
\begin{equation}
    \mu_a = 
    f_\text{mel} \mu_{a, \text{mel}} 
    + (1-f_\text{mel}) \mu_{a,\text{epi}},
\end{equation}
where $f_\text{mel}$ is the volume fraction of melanin. Absorbed radiation is converted to thermal energy, causing the skin to heat up. Melanin concentration varies across the population, causing some skin heats up more than others. The direct relationship between solar loading and melanin motivates the use of a colormeter for analyzing skin tone later.


\subsection{Problem Statement and Challenges}
% move to the method section???
In this work, we collect data during the cooling state and desire to recover the baseline state from a thermal image. 
Skin temperature is a time-dependent 3D field, as well as environmental variables.
However, a thermal camera can only measure the skin \textit{surface} temperature, $T(x,y) = u(x,y,z=0)$.
We can also define $T_0(x,y)=u_0(x,y,z=0)$ and $S(x,y,t)=s(x,y,z=0,t)$.
making it difficult to invert for skin temperature directly. 
However, there is a standard appearance for skin temperature so we can learn this using a machine learning model.
Our goal is to 
\begin{equation}
    f: T \rightarrow T_0, S
\end{equation}

which can be passed to existing forehead thermometers to estimate body temperature.

==> sections/thermal-features.tex <==
% A camera can only observe the skin surface, so it measures $u(x, y, t; z=0)$. Skin emissivity is near unity but it is still directional emitting.
% \begin{equation}
%     T_\text{cam} = \varepsilon(\phi(x,y), \theta(x,y)) u(x, y, z=0)
% \end{equation}
% Even though the camera does not exactly measure skin temperature, this is not a problem for previous works because they extract temperature from the forehead or inner canthus, which are relatively flat areas.

Our aim is to recover baseline skin temperature from a single thermal image. Input, Output and Assumptions of the problem.

With standard infrared thermometers, the problem of recovering baseline temperature is ill-posed: we cannot recover the baseline and transient from a single measurement. To recover the baseline, we can leverage data across two dimensions, time and space. 


\subsection{Solar Loading}
When a subject is solar loaded, their skin temperature is transient and the spatial solar loading pattern depends on the face geometry.
% so $\pdv{u}{t} > 0, s > 0, q_\text{ext} > 0$.
For \textit{solar loading}, $q_\text{ext}$ is a function of the solar power, $P_0$, and direction, $d$, of the sun, and the surface normals, $n$, and absorption coefficient, $\mu_a$, of the face.
Solar radiation incident on the skin is:
\begin{equation}
    P(x,y) = P_0 \, \mathbf{\ell}^\top \mathbf{n}(x,y).
\end{equation}
The amount of heat absorbed is proportional to skin color $\mu_a$:
\begin{equation}
    q_\text{ext}(\vecx) = P(x,y) e^{-\mu_a z}.
\end{equation}
During cooling, the skin temperature begins to return to the baseline after heat exposure. In this case, 
For cooling, $\pdv{u}{t} < 0, s > 0, q_\text{ext} = 0$.


\subsection{Spatial Solution}
% Current thermometers only use temperature at one location of the face to estimate body temperature. Even though camera-based IRTs will image the whole face, they extract only one measurement from the forehead or canthus. The discarded pixels, however, hold valuable information for determining temperature state.
% Empirically, baseline face temperature has a standard appearance: the forehead and inner eyes are hot, and the cheeks are nose are cooler. This is due to face vasculature, and vasculature is common to all humans.

Physiology-based thermal image processing focuses on deviations from the standard thermal features, such as for facial recognition and emotion classification. 
Such thermal features are usually hand-crafted, as is the case for thermal minutia points (TMP). 
As machine learning and specifically convolutional neural networks (CNNs) have been increasingly used to process human thermal imagery, the thermal features learned by the model are likely based on physiology but are less interpretable. 
In the following, we show how the structure of a CNN is conducive to learning physiological features and how this can correct solar loading.


\subsubsection{Bioheat Thermal Features}
The bioheat equation (\cref{eq:gov}) suggests a link between spatial and temporal patterns according to its formulation as a PDE. We will clarify how this is useful for our problem setting.
First we rewrite \cref{eq:gov} for the input data available in our problem setting: skin surface temperature, $T(x,y) = u(x,y,z=0)$:
\begin{align}
    \rho c \pdv{T}{t} 
    = k \nabla^2 T
    + B (T_c - T) 
    + q_m.
\end{align}
Subjects are screened upon entering a building so $q_\text{ext}=0$.

Recall that $\nabla^2$ operates in all spatial dimensions, $x,y,z$. The camera only sees the skin surface and only observes temperature gradients in the $x,y$ directions. Additionally, in a single-shot setting, $\pdv{T}{t}$ is also unknown.
Defining $\nabla_i^2 = \pdv[2]{}{i}$, we gather all the unknown derivatives on one side of the equation:
\begin{align}
    k\nabla_x^2 T + k\nabla_y^2 T + B(T_c - T)
    = \rho c \pdv{T}{t} - k\nabla_z^2 T - q_m.
\end{align}

$T$ is captured by the thermal camera and $T_0$ and $S$ are unknown, but do not appear in the equation. By definition, $T_0$ is stationary so $\pdv{T}{t} = \pdv{S}{t}$. We introduce $T_0$ by substituting $T = T_0 + S$ on the right hand side:
\begin{align}
    z &= k\nabla_x^2 T + k\nabla_y^2 T +  B(T_c - T) \label{eq:lhs} \\
     &= \rho c \pdv{S}{t} - k\nabla_z^2 S - k\nabla_z^2 T_0 - q_m. \label{eq:rhs} 
\end{align}
\cref{eq:lhs} depends on $T$, the input, and $T_c$, a subject-specific constant and $B$, spatially varying blood flow; $z$ is a filtered version of $T$ based on $B$.
The right hand side sums contributions from our two unknowns, $T_0$ and $S$.
$z$ is a representation of $T$ where the unknowns are separable according to \cref{eq:rhs}. 


\subsubsection{Learning Thermal Features}
This representation follows the structure of a encoder-decoder: an encoder $E(T)$ with learned weights, filters the input to a latent $z$, from which the decoder $D(z)$ recovers the desired output. 
It is clear that the encoder can be learned because $z$ is the sum of the 2D Laplacian and a blood term, and $B$ remains similar across all humans. 
The ability to learn the decoder is less clear, due to the partial derivatives.
However, since $T_0$ has a common appearance, the Laplacian across z has a common appearance too. 
The latent learned by a CNN is not exactly \cref{eq:lhs} because the latent is of size $n_d$ while $z$ is $m\times n$.


\subsection{Temporal Solution}
Our prior discussion centered on using spatial data to detect temperature transients. We may also use temporal data and the method for finding $T_0$ is more straightforward and has a closed form solution.
Since data is collected upon entry, a subject is cooling. If the cooling conditions are kept constant, the cooling temperature will be a decaying exponential that tends to the baseline \cite{Vollmer2009} \footnote{This relation is not a completely accurate description}:
\begin{equation}
    T_f(t) = a e^{-bt} + T_{f,0}.
    \label{eq:exponential}
\end{equation}
$T_f$ denotes forehead temperature.
In theory, we only need three temporal measurements to fit this curve and find the baseline. Unfortunately, the rate of cooling is not much larger than the camera noise floor, making it difficult to solve for the baseline even with minutes of data as we will see in \cref{sec:results}.


% The left hand size is some filtered version of $T$. 
% \begin{equation}
%     f_1(T) = f_2(T_0) + f_3(S)
% \end{equation}

% We approximate $f_1(T)$ using an encoder $E(T)\approx z$. Then $S, T_0$ can be calculated as follows and approximated by a decoder:
% \begin{align}
%     S = f_1^{-1} (z - f_2(T_0)) \approx D_1(z) \\
%     T_0 = f_2^{-1} (z - f_1(S)) \approx D_2(z).
% \end{align}


% Applying PBHE to the steady state case:
% \begin{equation}
%     0 = \pdv[2]{u_0}{x} + \pdv[2]{u_0}{y} + \pdv[2]{u_0}{z} + b(T_c - u_0) + m
% \end{equation}

% \begin{equation}
%     \pdv[2]{u_0}{z} + m = -\pdv[2]{u_0}{x} - \pdv[2]{u_0}{y} - b(T_c - u_0)
% \end{equation}


